Safety and Security: Experimental Validation of Encrypted Model Predictive Control

In this paper, we revisit the problem of an encrypted model predictive control (MPC) design, representing a significant challenge in the recent field of secure process control. Existing methods in secure optimization-based control are non-existent and even partial implementation fails to address the closed-loop system stability and recursive feasibility properties of the constrained MPC. To overcome these limitations, we propose a novel approach that utilizes a polynomial approximation of the optimal control law. This method evaluates the explicit control law within a fully homomorphic encryption framework, ensuring that the controller is securely deployed on any third-party or cloud-based platform, with both process data and controller coefficients protected. Experimental results from a laboratory-scale implementation and validation of the proposed privacy-aware control method demonstrate its advantages.

==> images/preamble.tex <==
\usepackage{cite}

%\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
%    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}


\usepackage{upgreek} % for greek letters
\usepackage{amsmath, mathtools, amssymb} % for math operations
\usepackage{amsfonts} % for math operations
\usepackage{graphicx} 
\usepackage{listings}
\usepackage{multirow}
\usepackage{dutchcal}
\usepackage{siunitx}
\usepackage{booktabs}
\usepackage{scalerel}
\usepackage{subfigure}
\usepackage{url}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\SetKwRepeat{Do}{do}{while}%

\newcommand{\pointout}[1]{\textcolor{red}{#1}}

\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\nint}[1]{\ensuremath\left\lfloor#1\right\rceil}

\newcommand{\ui}[2]{#1_{\text{#2}}}
\newcommand{\ei}[2]{#1^{\text{#2}}}

\newcommand{\pk}{\ui{k}{pub}}
\newcommand{\sk}{\ui{k}{pvt}}
\newcommand{\ek}{\ui{k}{eval}}

%\def\shrinkage{-2mu}
%\def\vecsign#1{\rule[1.6\LMex]{\dimexpr#1-2pt}{.001\LMpt}%
%	\kern-5.0\LMpt\mathchar"017E}
%\def\dvecsign#1{\rule{0pt}{7\LMpt}\smash{\stackon[-1.989\LMpt]{%
%			\SavedStyle\mkern-\shrinkage\vecsign{#1}}%
%		{\rotatebox{180}{$\SavedStyle\mkern-\shrinkage\vecsign{#1}$}}}}
%\def\dvec#1{\ThisStyle{\setbox0=\hbox{$\SavedStyle#1$}%
%		\def\useanchorwidth{T}\stackon[-4\LMpt]{\SavedStyle#1}{\,\dvecsign{\wd0}}}}
%\usepackage{stackengine,amsmath}
%\stackMath
\DeclareFontEncoding{LS1}{}{}
\DeclareFontSubstitution{LS1}{stix}{m}{n}
\DeclareSymbolFont{stixletters}{LS1}{stix}{m}{it}
\DeclareMathAccent{\cev}{\mathord}{stixletters}{"91}
\DeclareMathAccent{\vec}{\mathord}{stixletters}{"92}
\DeclareMathAccent{\vecev}{\mathord}{stixletters}{"95}

% MPC macro + packages
\newcommand{\Ts}{\ui{T}{s}}
\DeclareMathOperator{\interior}{int}
\usepackage{bbold}
\newcommand{\pnorm}{n}
\newcommand{\pdegree}{\kappa}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}{Definition}[section]
% \newtheorem{proof}{Proof}[section]
\newtheorem{proof}[theorem]{Proof}
\newtheorem{assumption}{Assumption}[section]
\newtheorem{problem}[theorem]{Problem}

%%-------------------------------------------------------
%% MACRO for tikz picture. DO NOT CHANGE ANYTHING !!!!!
\usepackage{tikz}
\usepackage{pgfkeys}
\usepackage{calc}
\usepackage{pgfplots}
\pgfplotsset{compat=1.17}
\usetikzlibrary{arrows}
\usetikzlibrary{calc}
\usepgflibrary{arrows}
\usetikzlibrary{positioning}
\usetikzlibrary{intersections}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{patterns,decorations.pathmorphing,decorations.markings}
\usetikzlibrary{external}
\usetikzlibrary{plotmarks}
\usetikzlibrary{arrows.meta}
\usepgfplotslibrary{patchplots}
\usepackage{grffile}
\usepgfplotslibrary{fillbetween}
\usepackage{xfrac}
%\tikzexternalize

\newcommand{\includetikz}[1]{%
\tikzifexternalizing{%
\def\DOIT{1}%
}{%
\IfFileExists{#1.pdf}{%
\includegraphics[scale=1]{#1.pdf}%
\def\DOIT{0}%
}{%
\def\DOIT{1}%
}%
}%
%
\if1\DOIT
%	\tikzsetnextfilename{mypic_#1}%
\tikzsetnextfilename{#1}
%   \filemodCmp{#1.tikz}{external/#1.log}%
%  {\tikzset{external/force remake=true}\input{#1.tikz}}
\input{#1.tikz}
\fi
}

% defines lengths for figure plotting
\newlength\figureheight
\newlength\figurewidth
%%  End of TikZ Macros
%%-------------------------------------------------------

\newcommand{\red}[1]{{\color{red}#1}}
